Lessons in VCR Repair: Compliance of Android App Developers with the California Consumer Privacy Act (CCPA)

The California Consumer Privacy Act (CCPA) provides California residents with a range of enhanced privacy protections and rights. Our research investigated the extent to which Android app developers comply with the provisions of the CCPA that require them to provide consumers with accurate privacy notices and respond to "verifiable consumer requests" (VCRs) by disclosing personal information that they have collected, used, or shared about consumers for a business or commercial purpose. We compared the actual network traffic of 109 apps that we believe must comply with the CCPA to the data that apps state they collect in their privacy policies and the data contained in responses to "right to know" requests that we submitted to the app's developers. Of the 69 app developers who substantively replied to our requests, all but one provided specific pieces of personal data (as opposed to only categorical information). However, a significant percentage of apps collected information that was not disclosed, including identifiers (55 apps, 80%), geolocation data (21 apps, 30%), and sensory data (18 apps, 26%) among other categories. We discuss improvements to the CCPA that could help app developers comply with "right to know" requests and other related regulations.

==> content/7_conclusion.tex <==
%-------------------------------------------------------------------------------
\section{Conclusion}
\label{sec:conclusion}
%-------------------------------------------------------------------------------
...

==> content/unused/6_related.tex <==
%-------------------------------------------------------------------------------
\section{Related Work}
%-------------------------------------------------------------------------------


Our work relates to prior studies that investigated the accuracy of disclosures made in privacy policies~\cite{andow2019policylint, okoyomon2019ridiculousness, wang2018guileak}, the efficacy of data subject access requests mechanisms~\cite{veys2021pursuing, di2019personal, di2022revisiting, kroger2020app}, and the potential privacy violations that exist in online systems, including mobile apps and web-based systems~\cite{nguyen2021share, reyes2018won, han2020price}. In~\cite{urban2019study}, data subject access requests were sent to 38 third-party organizations in an effort to evaluate how they comply with Article 15 of the GDPR, and the study showed that most failed to properly disclose all relevant data in their responses to the requests. Jacob et al.~\cite{kroger2020app} sent similar requests to 225 app developers over a period of four years and identified shortcomings in the processes developers followed to handle and respond to such requests that continued to exist even after GDPR was enforced. Similarly, the results of contacting 60 data controllers with data access requests in~\cite{ausloos2018shattering} highlighted the difficulty these controllers experienced with finding all relevant data needed to respond to such requests. The authors also emphasized the importance of automating the process of responding to DSARs and developing templates that data controllers can follow in order to reach a state of ``legal certainty'', where they can be assured that they are compliant with laws that provide users with the right to access their data. In a study that focused on app developers and website operators, Dominik and Jens~\cite{herrmann2016obtaining} observed higher response rates for data deletion requests compared to data subject access requests, and found that 20\% of the websites considered in the study adopted processes that can be abused to leak users' data to adversaries. In a number of other studies, researchers focused on examining whether businesses can be tricked into revealing subjects' data through impersonation and social engineering attacks~\cite{di2019personal, di2022revisiting, pavur2019gdparrrrr, cormack2016subject, boniface2019security}. Mariano et al.~\cite{di2019personal} proved the possibility of launching these types of attacks for a number of organizations by relying on information that is available to the public. In their follow-up work~\cite{di2022revisiting}, they proposed alternative approaches to authenticating data subjects that can help organizations prevent leaking their users' data when they respond to data access requests made by adversaries.  

In another line of work, researchers focused on studying the usability of data subject access request mechanisms from a number of different angles, including the ease of initiating the requests as well as the extent to which the content of the responses can be understood by average users~\cite{veys2021pursuing, wei2020twitter, habib2020s}. Veys et al.~\cite{veys2021pursuing} gathered insights from real users after asking them to submit DSARs to a number of service providers and identified issues with the format as well as the content of the responses which might render them \textit{inaccessible} to users. Wei et al.~\cite{wei2020twitter} leveraged data access requests submitted to Twitter to study how users perceive ad targeting and found that providing detailed explanations of how ads were targeted in the responses was more appreciated by users. 

Some authors have conducted studies that focused specifically on investigating potential compliance with the CCPA. For instance, a recent report from Consumer Reports has found that consumers struggled to opt-out of the sale of their personal information and were at least somewhat dissatisfied with the opt-out process 52\% of the time~\cite{mahoney2020california}. More recently, Nortwick and Wilson~\cite{van2022setting} found that many websites that are required to comply with CCPA either failed to provide users with options to request not selling their data to third parties or provided options that suffered from major usability issues.

The focus in other research studies has been on understanding privacy practices by analyzing disclosures made in privacy policies~\cite{harkous2018polisis, andow2020actions, wang2018guileak, zimmeck2019maps, zimmeck2016automated}. Some researchers proposed systems, such as POLICHECK~\cite{andow2020actions} and MAPS~\cite{zimmeck2019maps}, that automated the process of measuring the level of consistency between what is disclosed in privacy policies versus what can be observed by looking at network data flows~\cite{wang2018guileak, andow2020actions,zimmeck2019maps, zimmeck2016automated, slavin2016toward}. The literature also proposed systems such as Polisis~\cite{harkous2018polisis} and PI-Extract~\cite{bui2021automated} that automated the process of transforming privacy policy texts into more understandable formats. Linden et al.~\cite{linden2018privacy} found that disclosures made in privacy policies improved as a result enforcing the GDPR, but that more improvements would have to be made before they can be considered usable and transparent to end users.

To examine the extent to which mobile apps are complying with privacy regulations, researchers also relied on static and dynamic app analysis tools to identify potential legal violations at scale~\cite{reyes2018won, han2020price, feal2020angel, nguyen2021share, ren2018longitudinal}. These studies identified a range of deceptive data collection and transmission practices and highlighted the need for stronger enforcement actions by regulators. While prior work has examined apps' level of compliance with privacy regulations by looking into network data flows, privacy policy disclosure or responses to data subject access requests, our investigation compares the data obtained from all these three sources to evaluate the effect of enforcing the CCPA on developers' privacy practices. We believe that our work, therefore, is crucial in evaluating the overall efficacy of CCPA and its utility to mobile app users.

%Other studies have also found issues with similar privacy laws enacted earlier, such as GDPR in Europe, including evidence of non-compliance by app developers~\cite{zimmeck2019maps} and personal information leakage by abusing the GDPR ``right of access''~\cite{di2019personal}. 




%Our study will complement these findings by focusing specifically on the CCPA; in particular, we will examine the process of submitting a verifiable consumer request and compare the responses from app developers with the actual privacy practices that we identify through app and network analysis. 

==> content/unused/undisclosed_pii_old.tex <==
\begin{table*}[t]
\small\centering

\label{tab:undisclosed}
\begin{tabular}{lllll}
\hline
PII Category                    & PII Subcategory                   & PII Name                      & Example Value                     & App \#     \\ 
\hline\hline
Identifiers                     & App-Specific                      & Android ID                    & 7892f8834ddbf2df                          & 15           \\
                                &                                   & Miscellaneous                 & 1039977256339324001                       & 9           \\
                                & Device-Specific                   & AAID                          & 03140e43-9bb7-4ee4-97c6[...]              & 50          \\
                                &                                   & Miscellaneous                 & 1038453736229100022                       & 18           \\
                                &                                   & IMEI                          & 359677097304580                           & 2           \\
                                &                                   & SIM ID                        & 8901260853115626226                       & 2           \\
                                &                                   & IMSI                          & 310260851562622                           & 2           \\
                                &                                   & WIFI MAC                      & 58:CB:52:8B:C8:66                         & 1           \\
                                & Network-Specific                  & IP Address                    & 135.***.***.79                            & 21           \\
                                &                                   & Router SSID                   & *** of the ****                           & 9           \\
                                &                                   & Router MAC                    & 48:**:**:**:**:06                         & 8           \\
                                & User-Specific                     & App Username                  & schneider90christopher19                  & 4           \\
                                &                                   & Device Username               & schneider90\_device                        & 3           \\
\hline
Customer Records                &                                   & Postal Address                & 957 Green Causeway                        & 9           \\
                                &                                   & Phone Number                  & 323-***-8894                              & 5           \\
                                &                                   & Contacts List Information     & Scott Pratt                               & 4           \\
\hline
Protected Classifications       &                                   & Date of Birth                 & 20-May-1990                               & 4           \\
                                &                                   & Gender                        & Male                                      & 1           \\
\hline
Geolocation Data                & Coarse                            & GPS Coordinates               & *****                                     & 27           \\
                                &                                   & Zip Code                      & *****                                     & 2           \\
                                &                                   & City Name                     & *****                                     & 7           \\
                                & Precise                           & GPS Coordinates               & *****                                     & 15           \\
\hline
Sensory Data                    &                                   & Embedded Sensors Reading      & AK0991X                                   & 21           \\

Employment Information          &                                   & Company or Job                & Music Teacher                             & 4           \\

Education Information           &                                   & University Name               & Villanova University                      & 1           \\


\hline
\end{tabular}
\caption{Counts of Apps that Collected but not Disclosed Various PII}
\end{table*}

==> tables/ccpa_categories_1.tex <==
% \usepackage{array}


\begin{table*}
\small
\centering
\caption{Categories of Personal Information defined under the CCPA}
\begin{tabular}{>{\hspace{0pt}}m{0.2\linewidth}|>{\hspace{0pt}}m{0.7\linewidth}} 
\hline
Category                      & Description                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ 
\hline\hline
Identifiers                   & Identifiers such as a real name, alias, postal address, unique personal identifier, online identifier, IP address, email address, account name, social security number, driver’s license number, passport number, or other similar identifiers.                                                                                                                                                                                                                                            \\ 
\hline
Customer Records              & Customer records such as name, signature, social security number, physical characteristics or description, address, telephone number, passport number, driver’s license or state identification card number, insurance policy number, education, employment, employment history, bank account number, credit card number, debit card number, or any other financial information, medical information, or health insurance information.                                                     \\ 
\hline
Protected Classifications     & Characteristics of protected classifications under California or federal law such as age (40 years or older), race, color, ancestry, national origin, citizenship, religion or creed, marital status, medical condition, physical or mental disability, sex (including gender, gender identity, gender expression, pregnancy or childbirth and related medical conditions), sexual orientation, veteran or military status, genetic information (including familial genetic information).  \\ 
\hline
Commercial Information        & Records of personal property, products or services purchased, obtained, or considered, or other purchasing or consuming histories or tendencies.                                                                                                                                                                                                                                                                                                                                           \\ 
\hline
Biometric Information         & Genetic, physiological, behavioral, and biological characteristics, or activity patterns used to extract a template or other identifier or identifying information, such as, fingerprints, faceprints, and voiceprints, iris or retina scans, keystroke, gait, or other physical patterns, and sleep, health, or exercise data.                                                                                                                                                            \\ 
\hline
Internet Activity Information & Internet or other electronic network activity information such as browsing history, search history, or information regarding a consumer’s interaction with a website, application, or advertisement.                                                                                                                                                                                                                                                                                       \\ 
\hline
Geolocation Data              & Information such as physical location or movements.                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ 
\hline
Sensory Data                  & Audio, electronic, visual, thermal, olfactory, or similar information.                                                                                                                                                                                                                                                                                                                                                                                                                     \\ 
\hline
Professional Information      & Information such as current or past job history or performance evaluations.                                                                                                                                                                                                                                                                                                                                                                                                                \\ 
\hline
Education Information         & Education records directly related to a student maintained by an educational institution or party acting on its behalf, such as grades, transcripts, class lists, student schedules, student identification codes, student financial information, or student disciplinary records.                                                                                                                                                                                                         \\ 
\hline
Inferences                    & Inferences that can create a profile about a consumer reflecting the consumer’s preferences, characteristics, psychological trends, preferences, predispositions, behavior, attitudes, intelligence, abilities, or aptitudes.                                                                                                                                                                                                                                                              \\
\hline
\end{tabular}
\end{table*}

==> tables/name.tex <==
\begin{table*}[t]
\normalsize\centering
\caption{Different methods and PII types required to initialize or verify DSAR}
\label{tab:analysis}
\begin{tabular}{llll}
\hline
Method or PII Type & Initialize & Verify & Total \\ 
\hline
\hline
Email                                                                              & 32                                                   & 6                                                    & 38           \\
Account Authentication                                                             & 27                                                   & 11                                                    & 38           \\
Email Authentication                                                   & 5                                                    & 23                                                    & 28            \\
Full Name                                                                          & 25                                                   & 3                                                    & 28           \\
State of Residence                                                                 & 21                                                   & 0                                                    & 21           \\
Country of Residence                                                               & 14                                                   & 1                                                    & 15           \\
Street Address, City, or Zip Code                                                  & 12                                                   & 2                                                    & 14           \\
App-usage History                               & 2                                                    & 11                                                   & 13           \\
Names of Apps, Services, Brands                             & 10                                                   & 3                                                    & 13           \\
Username                                                                           & 3                                                    & 6                                                    & 9            \\
Phone Number                                                                       & 2                                                    & 5                                                    & 7            \\
Account, User, or Device ID                                                        & 1                                                    & 6                                                    & 7            \\
Google Advertising ID (AAID)                                                       & 0                                                    & 5                                                    & 5            \\
Certification under the Penalty of Perjury                                         & 5                                                    & 0                                                    & 5            \\
Signed Affidavit                                                                   & 0                                                    & 4                                                    & 4            \\
California Resident or Not                                                         & 4                                                    & 0                                                    & 4            \\
Current IP Address                                                                 & 2                                                    & 1                                                    & 3            \\
Phone Authentication                                                    & 0                                                    & 3                                                    & 3            \\
Date of Birth                                                                      & 2                                                    & 0                                                    & 2            \\
Photocopy of a Government-issued ID                               & 0                                                    & 2                                                    & 2            \\
ID.me                               & 0                                                    & 1                                                    & 1            \\
Call with a Company Representative                               & 0                                                    & 1                                                    & 1            \\
\hline
\end{tabular}
\end{table*}

==> tables/policy_categories.tex <==
\begin{table}
\small\centering
\caption{PII Categories Disclosed in Privacy Policies}
\begin{tabular}{>{\hspace{0pt}}m{0.398\linewidth}|>{\hspace{0pt}}m{0.213\linewidth}|>{\hspace{0pt}}m{0.173\linewidth}|>{\hspace{0pt}}m{0.144\linewidth}} 
\hline
Category                      &          & Collected \# & Shared \#  \\ 
\hline\hline
Identifiers                   & \#       & 79           & 75         \\
                              & $\alpha$ &              &            \\
Customer Records              & \#       & 72           & 63         \\
                              & $\alpha$ &              &            \\
Protected Classifications     & \#       & 47           & 38         \\
                              & $\alpha$ &              &            \\
Commercial Information        & \#       & 63           & 52         \\
                              & $\alpha$ &              &            \\
Biometric Information         & \#       & 9            & 6          \\
                              & $\alpha$ &              &            \\
Internet Activity Information & \#       & 79           & 72         \\
                              & $\alpha$ &              &            \\
Geolocation Data              & \#       & 70           & 61         \\
                              & $\alpha$ &              &            \\
Sensory Data                  & \#       & 53           & 44         \\
                              & $\alpha$ &              &            \\
Professional Information      & \#       & 29           & 24         \\
                              & $\alpha$ &              &            \\
Education Information         & \#       & 13           & 13         \\
                              & $\alpha$ &              &            \\
Inferences                    & \#       & 47           & 41         \\
                              & $\alpha$ &              &           
\end{tabular}
\end{table}

==> utils/heading.tex <==
% SET THESE OPTIONS FOR PETS 2023
\setcopyright{none}
\copyrightyear{2023}
\acmYear{2023}
\acmDOI{XXXXXXX.XXXXXXX}
\acmISBN{}
\acmConference[PoPETs]{Proceedings on Privacy Enhancing Technologies}{July 10--14, 2023}{Lausanne, Switzerland}
\settopmatter{printacmref=false,printccs=false}
